A Survey of Distributed Optimization Methods for Multi-Robot Systems

Distributed optimization consists of multiple computation nodes working together to minimize a common objective function through local computation iterations and network-constrained communication steps. In the context of robotics, distributed optimization algorithms can enable multi-robot systems to accomplish tasks in the absence of centralized coordination. We present a general framework for applying distributed optimization as a module in a robotics pipeline. We survey several classes of distributed optimization algorithms and assess their practical suitability for multi-robot applications. We further compare the performance of different classes of algorithms in simulations for three prototypical multi-robot problem scenarios. The Consensus Alternating Direction Method of Multipliers (C-ADMM) emerges as a particularly attractive and versatile distributed optimization method for multi-robot systems.

==> BLE_old.tex <==
	
	\subsection{Distributed Linear Least Squares Optimization}
	
	
	
	
	We can obtain the maximum a-posteriori (MAP) estimate from the optimization problem:
	\begin{equation}
	    \label{eq:trajectory_estimation}
	    \begin{aligned}
	    \min_x \quad & \norm{x_{0} - \mu_{0}}_{\Sigma_{0}^{-1}}^{2} + \sum_{t=1}^{T-1} \norm{x_{t+1} - Ax_{t}}_{Q^{-1}}^{2}  \\
	    & + \sum_{i=1}^{N} \sum_{t \in \mc{T}_i} \norm{y_{i,t} - Cx_{t}}_{R^{-1}}^{2} .
	    \end{aligned}
	\end{equation}
	% where robot $i$ makes observation $y_{i,t} \in \mathbb{R}^{m}$ of the target's trajectory $x_{t} \in \mathbb{R}^{n}$ and $\mu_{0}$ represents our estimate of the initial position of the target with $\Sigma_{0}$ representing the covariance (and our associated confidence) in this estimate. The summation over $i$ only involves robots which observe the agent at time $t$.
	
	Formulating \ref{eq:trajectory_estimation} as a distributed optimization problem requires introducing local variables $x_{i,t} \in \mathbb{R}^{n}$ representing robot $i$'s estimate of the targets trajectory at time $t$. Rewriting the optimization problem using these local variables yields the following equivalent distributed optimization problem:  
	\begin{equation}
	    \label{eq:trajectory_estimation_distributed}
	    \begin{aligned}
	    \min_{x} \quad & \sum_{i=1}^{N} \Big(\frac{1}{N}\sum_{t = 1}^{T-1}\norm{x_{i,t+1} - Ax_{i,t}}_{Q^{-1}}^{2} \\
	    & + \sum_{t \in \mc{T}_{i}} \norm{y_{i,t} - Cx_{i,t}}_{R^{-1}}^{2} + \frac{1}{N} \norm{x_{i,0} - \mu_{0}}_{\Sigma_0^{-1}}^{2} \Big) \\
	    \text{s.t.} \quad & x_{i,t} = x_{j,t} \quad \forall (i,j) \in \mc{E} \text{ and } t = 1,\cdots,T \: .
	    \end{aligned}
	\end{equation} 
	
	% We assign $Q_{i,t} = Q_{t}$ and $\Sigma_{i,0} = \Sigma_{0}$ for $i = 1,\cdots,N$, and robot $i$ observes the target at time instances in $\mc{T}_{i}$. 
	We can express the objective function of the trajectory estimation problem \eqref{eq:trajectory_estimation_distributed} as $\mc{L} = \sum_{i=1}^{N} \mc{L}_{i}$ where robot $i$ has access to variables and data contained in $\mc{L}_{i}$ and can therefore compute its local gradients.
	
	The cost function in \ref{eq:trajectory_estimation_distributed} can be rewritten, using the concatenated versions of $x_{i,t}$ and $y_{i,t}$ for all $t=1,\cdots,T$ as $x_i$ and $y_i$ respectively, as 
	
	\begin{equation}
	    \label{eq:trajetory_estimation_blocks}
	    \begin{aligned}
	    \min_x \quad & \sum_{i=1}^N \norm{z_i - H_i x_i}_{W_i^{-1}}^2 \\
	    \text{s.t.} \quad & x_i = x_j \quad \forall (i,j) \in \mc{E}
	    \end{aligned}
	\end{equation}
	
	where $z_i = [\mu_0^T, y_i^T]^T$, $G_i \in \mathbb{R}^{|\mc{T}_i| \times T}$ is a matrix that has one-hot rows that correspond to each $t \in \mc{T}_i$, 
	\begin{align*}
		&P_{i} = \left[\begin{array}{cccc}
	        I       & \mbf{0}        & \mbf{0}      & \mbf{0} \\
	        -A      & I        & \mbf{0}      & \mbf{0} \\
	        \mbf{0} & -A       & I            & \mbf{0} \\
	        \vdots  & \ddots   & \ddots       & \ddots \\
	        \mbf{0} & \mbf{0}  & -A            & I 
	        \end{array}\right], \quad
	        \tilde{C}_i = G_i \otimes C, \\
	    &W_i = \text{diag}\Big(\Sigma_0, \{Q_t\}_{t=1}^T, \{R_t\}_{t \in \mc{T}_i}\Big), \quad
		H_{i} = \left[\begin{array}{c}
	        P_{i} \\ \tilde{C}_i
	        \end{array}\right]. \hspace{2em}    
	\end{align*}
	
%	where $D = [I,\mbf{0},\cdots,\mbf{0}] \in \mathbb{R}^{n\times n*(T+1)}$,
%	\begin{align*}
%	&G_{i} = \left[\begin{array}{c}
%	        P_{i} \\ C_{i}
%	        \end{array}\right], \hspace{2em}
%	H_{i} = \left[\begin{array}{cc} {
%	        Q_{i} & \mbf{0} \\ \mbf{0} & R_{i} }
%	        \end{array}\right] \\
%	&P_{i} = \left[\begin{array}{cccc}{
%	        -A      & I        & \mbf{0}      & \mbf{0} \\
%	        \mbf{0} & -A       & I            & \mbf{0} \\
%	        \vdots  & \ddots   & \ddots       & \ddots \\
%	        \mbf{0} & \mbf{0}  &-A            & I }
%	        \end{array}\right]
%	\end{align*}
%	and the diagonal matrix $Q_{i} \in \mathbb{R}^{nT \times nT}$ with $NQ_{i,t}$ on its diagonal, ${C_{i} \in \mathbb{R}^{m|\mc{T}_{i}| \times n|\mc{T}_{i}|}}$ contains the observation matrix $C_{i,t}$, and $R_{i} \in \mathbb{R}^{m|\mc{T}_{i}| \times m|\mc{T}_{i}|}$ has $R_{i,t}$ on its diagonals for $t \in \mc{T}_{i}$. 
%	
%	\begin{equation}
%	    \label{eq:trajectory_estimation_gradient}
%	    \nabla \mc{L}_{i}(x_{i}) = 2G_{i}^{T}H_{i}^{-1}G_{i}x_{i} - 2(C_{i}^{T}R_{i}^{-1}y_{i} + D^{T}\Sigma_{i,0}^{-1}\mu_{0})
%	\end{equation}
    In simulation the target has Dubin's car dynamics, and is orienting towards specific goal points in the environment. However, we approximate the dynamics of the target as a single integrator autonomous system. This assumption reflects a scenario wherein the robots cannot observe the control signal of the target, and must use linear approximations to simplify the non-linear dynamics of the target. As an aside, non-linear target models are addressed in \ref{sec:example3}. 
    
    The state of the target is modeled by the robots as it's Cartesian position and respective velocities; $x \in \mathbb{R}^{4}$. With a small sampling interval $\del{t}$, we ignore the orientation terms in $A$ and approximate the dynamics of the target using
    \begin{align*}
        \label{eq:target_dynamics_A}
        A = \left[\begin{array}{cccc} 
        1 & 0 &  \del{t} & 0  \\
        0 & 1 &  0 & \del{t}  \\
        0 & 0 &  1 & 0 \\
        0 & 0 &  0 & 1 \\
        \end{array}\right]
    \end{align*}
    where $A \in \mathbb{R}^{4 \times 4}$. For this problem, we selected $Q = 0.05 \: I$ to reflect the approximation of the target's dynamics in $A$.
    
    We assume each robot knows its position and observes the position of the target using a depth camera to extract the relative position and orientation of the target in its field of view with 
    \begin{align*}
        %\label{eq:robot_observations}
        C_{i,t} = \left[\begin{array}{cccc} 
        1 & 0 & 0 & 0   \\
        0 & 1 & 0 & 0  
        \end{array}\right]
    \end{align*}
    where $C_{i,t} \in \mathbb{R}^{2 \times 4}$ and $t \in \mc{T}_{i}$.
    
    \begin{figure}[ht]
        \centering
        \includegraphics[width=\columnwidth]{figures/schem_ble.png}
        \caption{Distributed linear estimation problem setup. The black nodes indicate robot position, and black lines indicate edges in the communication graph. The gray shaded region shows the sensing range for robot 1, and magenta points are observations made by robot 1 of the target. The green trajectory is the local estimate made by robot 1 with no communication and only its own observations. The orange trajectory shows the centralized estimate found by taking into account observations made by all of the robots.}
        \label{fig:linear_est_schematic}
    \end{figure}   
    Figure \ref{fig:linear_est_schematic} shows a graphical representation of this linear estimation problem. Since this optimization problem is convex, all of the methods featured in this comparison converge to the centralized solution.
    
    The goal of this simple linear estimation example is to provide insight into two key characteristics of all distributed optimization algorithms which are convergence as a function of both computation and communication time, and stability of methods with respect to choice of hyper parameters. 

    There are a number of ways to characterize error when analysing a distributed optimization algorithm. In this work we define error at a given time as the Mean Squared Error (MSE) of the individual solutions with respect to the centralized solution or
    \begin{equation}
        %\label{eq:average_error}
        \begin{aligned}
            \text{Error}(x_1, \cdots, x_N) = \frac{1}{N} \norm{x_i - x^*}_2^2
        \end{aligned}
    \end{equation}
    where $x^*$ is the centralized solution. 
    
    It is common in the distributed optimization literature to provide a result and perform comparisons based on the the reduction in MSE per update of the decision variable of the distributed optimization algorithm. However, when comparing distributed optimization algorithms comparisons on the basis of MSE reduction per iteration can often skew results, and does not accurately reflect the total execution time of these algorithms. For example, methods like NN-P require a ``nested" communication loop that is not accounted for in a per iteration comparison, and similarly ADMM requires a local optimization step that depending on the local cost function can greatly increase computation time. It's clear that in real world application both communication time, and local computation time contribute to the overall execution time of these algorithms. Conveniently because the DLLS problem is convex and a globally optimal, centralized solution is available then we propose comparing algorithms based on a resource-weighted cost that factors in both communication and computation time.
    
    The resource-weighted cost represents the total time required for a distributed optimization algorithm to converge below an acceptable MSE given some arbitrary computation and communication capability:
    
    \begin{align*}
            \text{cost}_\lambda = \frac{t_{cp} + \lambda t_{cm}}{1 + \lambda} 
    \end{align*}
    where $t_{cp}$ is the sum of the time spent by all robots performing local computations, $t_{cm}$ is the time spent by all robots communication with their neighbors, and $\lambda$ is a scaling factor that weights communication to computation resource capability. Communication time is estimated based on the total number of floating point values passed during execution. The scalar $\lambda$ represents the ratio between time required for communication versus time required for computation. As an example, a network of robots connected via a 5G cellular network would require significantly less time to communicate the same amount of data versus the same network of robots connected via a low power radio network, and the same can be said for local computation capability. Sweeping across $\lambda$ corresponds to a pass over the range of possible network configurations. 
    
    Figure \ref{fig:BLE_surf} shows the inverted cost surfaces of a logarithmic sweep across problem dimension $n$, and network scaling factor $\lambda$. The topology of this surface is highly problem parameter dependent, and should be interpreted as a guide for understanding the trade-offs inherent to choosing a distributed optimization algorithm. In this case, ADMM dominates both EXTRA and DIGing in both sweep dimensions, and EXTRA is most competitive in scenarios where the decision variable dimension is smaller and communication is ``cheap".   
    
     \begin{figure}[ht]
        \centering
        \includegraphics[width=\columnwidth]{figures/comp_ble.png}
        \caption{Scaled cost comparison of distributed optimization algorithms on a distributed linear least squares problem. }
    \end{figure}   
    
	We note that convergence of distributed subgradient and dual averaging methods depend significantly on the weighting matrices and descent step sizes used in these methods. To ensure a fair comparison, we selected the gradient descent step size that yielded fastest convergence for each method in a given problem. In our evaluation, we used these parameters in \textbf{(table note)}. Consensus ADMM showed a lower sensitivity to the penalty parameter. Nonetheless, we selected the penalty parameter which yielded fastest convergence.
	
	We examine each method on a range-limited communication network where each robot communicates with other roots within a specified communication range and a chain network where each robot communicates with at most two robots, representing a sparsely-connected communication graph. We select a communication range that preserves network connectivity, satisfying the assumptions required for convergence of these methods. We randomly generate the communication graph in each problem. 

